What are the Desired Characteristics of Calibration Sets? Identifying Correlates on Long Form Scientific Summarization

Summarization models often generate text that is poorly calibrated to quality metrics because they are trained to maximize the likelihood of a single reference (MLE). To address this, recent work has added a calibration step, which exposes a model to its own ranked outputs to improve relevance or, in a separate line of work, contrasts positive and negative sets to improve faithfulness. While effective, much of this work has focused on how to generate and optimize these sets. Less is known about why one setup is more effective than another. In this work, we uncover the underlying characteristics of effective sets. For each training instance, we form a large, diverse pool of candidates and systematically vary the subsets used for calibration fine-tuning. Each selection strategy targets distinct aspects of the sets, such as lexical diversity or the size of the gap between positive and negatives. On three diverse scientific long-form summarization datasets (spanning biomedical, clinical, and chemical domains), we find, among others, that faithfulness calibration is optimal when the negative sets are extractive and more likely to be generated, whereas for relevance calibration, the metric margin between candidates should be maximized and surprise--the disagreement between model and metric defined candidate rankings--minimized. Code to create, select, and optimize calibration sets is available at https://github.com/griff4692/calibrating-summaries

==> ckpt/intro.tex <==
Traditionally, summarization models have been trained to maximize the likelihood of gold-standard references. This training paradigm introduces an exposure bias in that, during training, the model is not exposed to the metrics on which it is evaluated. Without being able to calibrate its own predictions with metrics, models are more prone to produce summaries with irrelevant or repetitive content \citep{zhao2022calibrating}, or mis-represent the source text \citep{maynez-etal-2020-faithfulness}.

% Directly optimizing metrics with reinforcement learning can be effective \citep{paulus2017deep} yet is difficult to optimize \citep{nan-etal-2021-improving}.

Calibration offers a flexible and effective set of methods to remedy this exposure bias by explicitly directing a model not to produce low quality summaries. By varying how candidate sets are constructed and optimized, an extra calibration step can unlock large gains in relevance (via ROUGE \citep{simcls, liu-etal-2022-brio}) and faithfulness \citep{nan-etal-2021-improving, cliff}.

Yet, much of this work has addressed the \emph{how} question--how to generate candidates \citep{cliff} and how to define effective calibration objectives \citep{zhao2022calibrating}. Instead, we seek answers to the \emph{why} question--what are the underlying characteristics of effective calibration sets, and conversely, what makes a bad set? To accomplish this research goal, we implement a diverse set of existing methods for constructing candidate summaries and pool them together. From a large candidate set, we implement different filtering strategies for set selection which target specific characteristics.


Additionally, the current research has focused on single-document news summarization. We seek to broaden and pressure test recent advances in contrastive fine-tuning by experimenting on four long-form, scientific, highly specialized corpora in which metrics, i.e., faithfulness, are non-trivial to define, capture, and categorize \citep{mckeown-keynote}.

\ganote{Chemistry Dataset Note and why it's interesting.}
\jsnote{Contains substantial jargon - provides the opportunity to build both large (factual misrepresentations) and small (minor jargon swaps) contrastive examples? Naturally coupled pairs of human-written texts (paper bodies) and summaries (abstracts)? Cover an area of direct practical concern?}

The primary contributions of this work are to: 1) benchmark recently proposed methods for creating, selecting, and optimizing contrast sets on three scientific long-form datasets; 2) conduct extensive experiments to better understand the underlying characteristics of contrast sets; 3) design methods which exploit these correlates to efficiently and effectively optimize contrast sets; 4) release a new abstract generation corpus which was scraped from the Open Access subsets of eight chemical journals.
